Computing Graph Neural Networks: A Survey from Algorithms to Accelerators

Graph Neural Networks (GNNs) have exploded onto the machine learning scene in recent years owing to their capability to model and learn from graph-structured data. Such an ability has strong implications in a wide variety of fields whose data is inherently relational, for which conventional neural networks do not perform well. Indeed, as recent reviews can attest, research in the area of GNNs has grown rapidly and has lead to the development of a variety of GNN algorithm variants as well as to the exploration of groundbreaking applications in chemistry, neurology, electronics, or communication networks, among others. At the current stage of research, however, the efficient processing of GNNs is still an open challenge for several reasons. Besides of their novelty, GNNs are hard to compute due to their dependence on the input graph, their combination of dense and very sparse operations, or the need to scale to huge graphs in some applications. In this context, this paper aims to make two main contributions. On the one hand, a review of the field of GNNs is presented from the perspective of computing. This includes a brief tutorial on the GNN fundamentals, an overview of the evolution of the field in the last decade, and a summary of operations carried out in the multiple phases of different GNN algorithm variants. On the other hand, an in-depth analysis of current software and hardware acceleration schemes is provided, from which a hardware-software, graph-aware, and communication-centric vision for GNN accelerators is distilled.

==> tables/accelerators-old.tex <==

% \begin{table*}
%     \centering
%     \renewcommand{\arraystretch}{0.9}
%     \caption{Background Literature: GNN Specific Accelerators}
%     \begin{tabular}{|>{\centering\arraybackslash}p{0.2cm}|>{\centering\arraybackslash}p{5.5cm}|>{\centering\arraybackslash}p{11cm}|} \hline
%          & \textbf{Study} & \text{Contributions} \\ \hline
%         \textbf{1.} & EnGN: A High-Throughput and Energy-Efficient Accelerator for Large Graph Neural Networks \cite{EnGN} & \begin{itemize}
%             \item Provisions a high throughput and energy efficient methodology for \acrshort{gnn} inference phase acceleration for all \acrshort{gnn} models  
%             \item Provisions a complete architectural layout for the \acrshort{gnn} accelerator, that can process large graphs  
%             \item Provisions a detailed analysis and comparison with the state of the art methods in \acrshort{gnn} acceleration on the basis of throughput and energy consumption, and shows magnitudes of orders of improvement 
%             \item Provisions additional points of improvements through tiling, scheduling as well as analysis of the graph structure 
%         \end{itemize} \\ \hline
%         \textbf{2.} & HyGCN: A GCN Accelerator with Hybrid Architecture \cite{Yan2020} & \begin{itemize}
%             \item Presents a hybrid two stage architecture for \acrshort{gcn} acceleration
%             \item The presented \acrshort{gcn} accelerator is for the inference stage in the corresponding \acrshort{gnn} model  
%             \item Presents optimization to the accelerator via advanced graph partitioning approaches, such as sparsity awareness
%             \item Additional provisions have also been defined, wherein latency and energy aware task pipelining strategies have been specified 
%             \item An analysis based on memory bandwidth utilization, energy consumption and speedup compared to state of the art approaches, i.e., PyG-\acrshort{cpu} and \acrshort{gpu}, has been provided. 
%         \end{itemize} \\ \hline
%         \textbf{3.} & AWB-GCN: Accelerating Graph Convolutional Networks through Runtime Workload Rebalancing  \cite{AWB} %AWB-GCN: A Graph Convolutional Network Accelerator with Runtime Workload Rebalancing \cite{AWB}
%         & \begin{itemize}
%             \item An acceleration architectural framework for \acrshort{gcn}s has been provided 
%             \item Primary focus is on mediating the loads on the various processing elements catering to the \acrshort{gcn} acceleration
%             \item The basis of such a strategy is to mitigate the workload imbalance created by the extreme sparsity present in graph data structures, thus enabling speedup of the entire process
%             \item The concept of \acrfull{spmm} has been utilized
%             \item Local workload imbalance management approaches and remote workload imbalance management, i.e., a global workload imbalance management, approach has been provisioned
%             \item Evaluation of the inference latency and energy efficiency with state of the art implementations depicts orders of magnitude improvement
%         \end{itemize} \\ \hline    
%         \textbf{4.} & NeuGraph: Parallel deep neural network computation on large graphs \cite{Ma2019} & \begin{itemize}
%             \item Provisions a generic parallel processing framework, NGra, for the \acrshort{gnnpl}
%             \item Provisions a method to express the \acrshort{dnn}s as graph operation stages, i.e., \textit{Scatter}, \textit{ApplyEdge}, \textit{Gather}, and \textit{ApplyVertex}
%             \item Presents an automatic graph partitioning as well as a chunk centric stream processing methodology, which takes into account data locality, data movement, and overlapping of parallel processing and data movement operations. 
%             \item Comparative analysis based on speedup factor with baseline methods using TensorFlow reveals possible enhancement of upto 4$\times$
%         \end{itemize}   \\ \hline
        
%      \end{tabular}
%     \label{tab2}
% \end{table*}


==> tables/inefficiencies.tex <==

%\begin{table*}
%    \centering
%    \caption{Accelerators: Weakness Analysis}
%    \begin{tabular}{|m{3cm}|m{12cm}|} \hline
%         \textbf{Accelerator} & \textbf{Key weaknesses} \\ \hline
%             EnGN & \begin{itemize}
%            \item The data movement in the ring-edge-reduce aggregation stage forces the data to permute a fixed number of times regardless the tile size, which leaves room for optimization.
%            \item The dataflow makes it difficult to accommodate varying-size feature vectors.
%            \end{itemize} \\
%            \hline
%             HyGCN & \begin{itemize} 
%             \item Having separate cores for aggregation and combination requires an unnecessary data movement between those.
%             \item Certain inter-phase synchronization is needed to avoid latency problems. \end{itemize} \\ \hline
%             AWB-GCN & \begin{itemize} 
%             \item No specific aggregation strategy to avoid loading a sparse matrix, such as the adjacency matrix. 
%             \item The aggregation dataflow is not aiming at minimizing data movement. \end{itemize} \\ \hline
%             Hardware acceleration of GNN & %\begin{itemize} 
             %\item The dataflow in their tiled architecture is not optimized to minimize overall energy expense, but rather to work in such coupled blocks scheme. 
            % \item Only tile-to-tile links are available, which can introduce latency penalties.\end{itemize} \\ \hline
             %NeuGraph & \begin{itemize} 
             %\item Not an ASIC implementation.
             %\item Ring-based dataflow can become sub-optimal.
             %\end{itemize} \\ \hline 
             %Reducing Communication in GNN Training & \begin{itemize} 
             %\item Methodology not explored yet on GNN accelerator designs.
             %\end{itemize} \\ \hline 
             
   % \end{tabular}
    
   % \label{tab_accel_inefficiencies}
%\end{table*}

